Unified Conversational Recommendation Policy Learning via Graph-based Reinforcement Learning

Conversational recommender systems (CRS) enable the traditional recommender systems to explicitly acquire user preferences towards items and attributes through interactive conversations. Reinforcement learning (RL) is widely adopted to learn conversational recommendation policies to decide what attributes to ask, which items to recommend, and when to ask or recommend, at each conversation turn. However, existing methods mainly target at solving one or two of these three decision-making problems in CRS with separated conversation and recommendation components, which restrict the scalability and generality of CRS and fall short of preserving a stable training procedure. In the light of these challenges, we propose to formulate these three decision-making problems in CRS as a unified policy learning task. In order to systematically integrate conversation and recommendation components, we develop a dynamic weighted graph based RL method to learn a policy to select the action at each conversation turn, either asking an attribute or recommending items. Further, to deal with the sample efficiency issue, we propose two action selection strategies for reducing the candidate action space according to the preference and entropy information. Experimental results on two benchmark CRS datasets and a real-world E-Commerce application show that the proposed method not only significantly outperforms state-of-the-art methods but also enhances the scalability and stability of CRS.

==> backup.tex <==

\begin{figure*}
\setlength{\abovecaptionskip}{2pt}   
\setlength{\belowcaptionskip}{2pt}
\centering
\includegraphics[width=\textwidth]{review.pdf}
\caption{Illustration of policy learning frameworks for IRS and CRS, including CRM~\cite{sigir18-crm}, EAR~\cite{wsdm20-ear}, and SCPR~\cite{kdd20-scpr}.}
\label{review}
\vspace{-0.5cm}
\end{figure*}


\section{Introduction}
Conversational recommender systems (CRS) aim to learn user's preferences and make recommendations through interactive conversations~\cite{cikm18-saur,wsdm20-ear,nips18-redial}. 
Since it has the natural advantage of explicitly acquiring user's preferences and revealing the reasons behind recommendation, CRS has become one of the trending research topics for recommender systems and is gaining increasing attentions. 
To study it, different problem settings of CRS have been proposed, either from the perspective of dialog systems, being a variation of task-oriented dialog~\cite{nips18-redial,coling2020-topic-crs,acl20-muulti-type-crs},  or from the perspective of recommender systems, being an enhanced interactive recommender system (IRS)~\cite{sigir18-crm,kdd18-q&r,wsdm20-ear}. 
In this work, we study the multi-round conversational recommendation (MCR) setting~\cite{sigir18-crm,wsdm20-ear}, where the system asks questions about  users' preferences on certain attributes or makes recommendations multiple times, and the goal is to find the target items to recommend with the minimum number of interactions. 

Unlike traditional recommender systems~\cite{icdm10-fm,www17-mf} or interactive recommender systems~\cite{wsdm2020-irs-rl,sigir20-graph-irl}, which mainly focus on solving the problem of which items to recommend, there are generally the other two core research questions for CRS~\cite{sigir20-tutorial}, including what questions to ask and when to ask or recommend.
Recent works demonstrate the importance of interactivity of asking clarifying questions in CRS~\cite{kdd16-convbandit,cikm18-saur,sigir20-qrs}.
%\citet{kdd16-convbandit} develop a preference elicitation framework to identify which questions to ask a cold-start user for quickly learning their preferences. 
%\citet{cikm18-saur} propose a unified model for asking aspect-based questions as well as making recommendation based on text matching. 
%\citet{sigir20-qrs} propose a question-based recommendation method to ask questions based on extracted descriptive terms and update user preferences based on collaborative filtering. 
More importantly, deciding when to ask or recommend is the key to coordinating conversation and recommendation for developing an efficient CRS~\cite{sigir18-crm,wsdm20-ear,kdd20-scpr}.


In MCR scenario, the CRS is typically formulated as a multi-step decision-making process and solved by reinforcement learning methods for policy learning~\cite{sigir18-crm,wsdm20-ear,kdd20-scpr}. As shown in Figure~\ref{review}(a), RL-based interactive recommender systems is only required to learn the policy to decide what items to recommend. However, the situation is more complicated in CRS, since there are two components to be combined into a single framework~\cite{arxiv20-crs}, i.e., conversation and recommendation components. \citet{sigir18-crm} and \citet{wsdm20-ear} employ policy gradient~\cite{nips99-pg} to improve the strategies of when and what attributes to ask, while the recommendation is made by an external recommendation model. In order to reduce the action space in policy learning, the state-of-the-art method in MCR~\cite{kdd20-scpr} only considers to learn the policy of when to ask or recommend, while two isolated components are responsible for the decision of what to ask and what to recommend. The overview of these two kinds of CRS is presented in Figure~\ref{review}(b) and \ref{review}(c). 

Despite the effectiveness of these methods, there are some issues remained to be tackled for real-world applications: 
(i) It is lack of scalability and generality to different domains or applications, since there are three different decision-making processes to be considered in CRS, including what attributes to ask, what items to recommend, and when to ask or recommend. It requires extra efforts to train an offline recommendation model~\cite{kdd20-scpr,wsdm20-ear} or pretrain the policy network with synthetic dialogue history~\cite{wsdm20-ear,sigir18-crm}.
(ii) The policy learning is hard to converge, since the conversation and recommendation components are isolated and lack of mutual influence  during the training procedure.


In this work, we formulate the aforementioned three separated decision-making processes in CRS as a unified policy learning problem for simplifying the CRS framework as well as bridging the gap between the recommendation and conversation components during the training procedure. 
Such unified conversational recommendation policy learning (UCRPL) aims at learning a unified policy to decide the action, either ask an attribute or recommend items, at each conversation turn to maximize the cumulative utility over the whole MCR process. The overview of the proposed unified policy learning for CRS is depicted in Figure~\ref{overview}. 
However, the UCRPL comes along with two challenges: (i) How to systematically combine conversation and recommendation components for unified policy learning? (ii) How to deal with sample efficiency issues? As the action space becomes overwhelmingly large in UCRPL, including all available attributes and items, it requires tremendous amount of interaction data to learn the best policy. 
Fortunately, the graph structure has the natural advantage of capturing the rich correlated information among different types of entities, which enables to discover collaborative user preferences towards attributes and items. 
Thus, we can leverage the graph structure to integrate the recommendation and conversation components as an organic whole, where the conversation session can be regarded as a sequence of nodes maintained in the graph to dynamically exploit the conversation history for predicting the action at the next turn. 
On the other hand, although the connectivity of the graph can also be used to eliminate invalid actions by path reasoning~\cite{kdd20-scpr}, there are still tremendous amount of candidates left for action searching. Since users are not likely to be interested in all items and attributes, we can focus on the potentially important candidates to improve the sample efficiency of UCRPL.

\begin{figure}
\setlength{\abovecaptionskip}{2pt}   
\setlength{\belowcaptionskip}{2pt}
\centering
\includegraphics[width=0.3\textwidth]{overview.pdf}
\caption{Illustration of unified policy learning for CRS.}
\label{overview}
\vspace{-0.5cm}
\end{figure}

To this end, we propose a novel and adaptive graph-based reinforcement learning framework, namely \textbf{UNI}fied \textbf{CO}nversational \textbf{R}ecomme\textbf{N}der (\textbf{UNICORN}). Specifically, due to the evolving nature of CRS, we leverage a dynamic weighted graph to model the changing interrelationships among users, items, and attributes during the conversation, and consider a graph-based Markov Decision Process (MDP) environment for simultaneously handling the decision-making of recommendation and conversation. 
Then we integrate graph-enhanced representation learning and sequential conversation modeling for modeling dynamic user preferences towards items and attributes.  
In addition, two simple yet effective action selection strategies are designed to handle the sample efficiency issue. Instead of enumerating the whole candidate item and attribute set, we adopt preference-based item selection and weighted entropy-based attribute selection strategies to only consider potentially important actions. 




In summary, the contributions of this paper are as follows:
\begin{itemize}[leftmargin=*,topsep=4pt]
    \item We formulate three separated decision-making processes in conversational recommender systems, including when to ask or recommend, what to ask, and what to recommend, as a unified conversational recommendation policy learning problem.
    \item To tackle UCRPL problem, we propose a novel and adaptive reinforcement learning framework, namely \textbf{UNI}fied \textbf{CO}nversational \textbf{R}ecomme\textbf{N}der (\textbf{UNICORN}), based on dynamic weighted graph. To handle the sample efficiency issue, we further design two simple but effective action selection strategies. 
    \item We construct a new real-world conversational recommendation dataset in E-Commerce scenario. Experimental results show that the proposed method significantly outperforms state-of-the-art CRS methods across four benchmark datasets and the real-world E-Commerce application. 
\end{itemize}

%\textbf{UNI}fied \textbf{CO}nversational \textbf{R}ecommendatio\textbf{N} policy learning (UNICORN)




\section{Related Works}

\textbf{Conversational Recommendation.}
Based on the problem settings, current CRS studies can be categorized into four directions~\cite{sigir20-tutorial}: 
(1) Exploitation-Exploration Trade-offs for
Cold-start Users~\cite{kdd16-convbandit,www20-convbandit}. These approaches leverage bandit approaches to balance the exploration and exploitation trade-offs for cold-start users in conversational recommendation scenarios. 
(2) Question-driven Approaches~\cite{cikm18-saur,sigir20-qrs,kdd18-q&r} aim at asking questions to users to get more information about their preferences, which is often addressed as ``asking clarification/clarifying question".  (3) Dialogue Understanding and Generation~\cite{kdd20-redial-kg,nips18-redial,coling2020-topic-crs,acl20-muulti-type-crs}. These studies focus on how to understand a user’s preferences and intentions from their utterances and generate fluent responses so as to deliver natural and effective dialogue actions.  (4) Multi-round Conversational Recommendation~\cite{sigir18-crm,wsdm20-ear,kdd20-scpr}. Under this problem setting, the system asks questions about the user’s preferences or makes recommendations multiple times, with the goal of  achieving engaging and successful recommendations with fewer turns of conversations. Among these problem settings, we target at the MCR problem. 



\noindent\textbf{RL in Recommendation.}
Reinforcement learning (RL) has been widely introduced into recommender systems due to its advantage of considering users' long-term feedbacks~\cite{www18-rl-newsrec,kdd18-rl-negativefeedback}.
RL-based recommendation formulates the recommendation procedure as an MDP of the interactions between the user and a recommendation agent, and employ RL algorithms to learn the optimal recommendation strategies~\cite{jmlr05,www18-rl-newsrec,kdd18-rl-negativefeedback}. Recent works on sequential recommendation~\cite{sigir20-rl-seqrec,sigir20-graph-rl-seqrec} and interactive recommendation~\cite{nips19-irs-rl,wsdm2020-irs-rl,sigir20-graph-irl} adopt RL to capture users' dynamic preferences for generating accurate recommendations over time. The goal of these approaches typically is to learn an effective policy for determining which items to recommend. As for conversational recommendation, RL-based methods are adopted to improve the strategies of the other two decision processes, including (i) which attributes to ask~\cite{sigir18-crm,wsdm20-ear} and (ii) when to ask or recommend~\cite{kdd20-scpr}. 
In order to  simplify the overall framework of MCR with better scalability and generality, we formulate these three core decision processes in conversational recommendation as a unified policy learning problem. 




\noindent\textbf{Graph-based Recommendation.}
Graph-based recommendation studies mainly leverage the graph structure for two purposes. The first one is to enhance the recommendation performance by graph-based representation learning, including exploiting the structure information for collaborative filtering~\cite{sigir19-graph-cf,recsys18-graph-cf,sigir20-lightgcn}, and adopting knowledge graph embeddings as rich content information~\cite{kdd16-kg,sigir18-kg}. Another group of studies model recommendation as a path reasoning problem for building explainable recommender systems~\cite{www19-explain,aaai19-explain}. Recent years have witnessed many successful applications of graph-based RL methods on different scenarios of recommender systems~\cite{www20-graph-rl,sigir19-graph-rl,sigir20-graph-gcqn,sigir20-graph-irl,sigir20-graph-rl-demo,kdd20-scpr}. 
For example, \citet{sigir19-graph-rl} employ a policy-guided graph search method to sample reasoning paths for recommendation, which is enhance with adversarial actor-critic for demonstration-guided path reasoning~\cite{sigir20-graph-rl-demo}. \citet{sigir20-graph-gcqn} and \citet{sigir20-graph-irl} employ graph convolutional network (GCN)~\cite{iclr17-gcn} for state representation learning to enhance the performance of traditional RL methods on recommendation policy learning. In this work, we study graph-based RL method for conversational recommendation scenario based on a dynamic weighted graph.




\section{Problem Definition}
\textbf{Multi-round Conversational Recommendation.}
In this work, we focus on the multi-round conversational recommendation (MCR) scenario~\cite{wsdm20-ear,kdd20-scpr}, in which the CRS is able to ask attributes or make recommendation multiple times. 

Specifically, on the system side, the CRS maintains a large set of items $\mathcal{V}$ to be recommended, and each item $v$ is associated with a set of attributes $\mathcal{P}_v$. In each episode, a conversation session is initialized by a user $u$ specifying an attribute $p_0$. Then, the CRS is free to ask the user's preference on an attribute selected from the candidate attribute set $\mathcal{P}_{\mathrm{cand}}$ or recommend a certain number of items (e.g., top-$K$) from the candidate item set $\mathcal{V}_{\mathrm{cand}}$. 
Following the assumptions from \citet{wsdm20-ear}, the user preserves clear preferences towards all the attributes and items. Thus, the user will respond accordingly, either accepting or rejecting the asked attributes or the recommended items. The CRS updates the candidate attribute and item sets and decides the next action based on the user response. 
The system-ask and user-respond process repeat until the CRS hits the target item or reaches the maximum number of turn $T$.

\noindent\textbf{Unified Conversational Recommendation Policy Learning.}
Multi-round conversational recommendation aims to make desired recommendations within a multi-round conversation session with the user. At each timestep $t$, according to the observation on past interactions, the CRS selects an action $a_t$, either ask an attribute or recommend an item. In return, the user expresses his/her feedback (accept or reject). This process repeats until the CRS hits the user-preferred items or reaches the maximum number of turn $T$. Such MCR process can be formulated as a Markov Decision Process (MDP). The goal of the CRS is to learn a policy $\pi$ maximizing the cumulative utility over the whole MCR process as
\begin{equation}
    \pi^*=\argmax\nolimits_{\pi\in\Pi}\mathrm{E}\left[\sum\nolimits_{t=0}^Tr(s_t,a_t)\right],
\end{equation}
where $s_t$ is the state representation learned from the system state and the conversation history, $a_t$ is the action that the agent takes at timestep $t$, and $r(\cdot)$ is the intermediate reward, abbreviated as $r_t$.



\section{Method}\label{sec:method}
\begin{figure*}
\setlength{\abovecaptionskip}{2pt}   
\setlength{\belowcaptionskip}{2pt}
\centering
\includegraphics[width=\textwidth]{ucrpl.pdf}
\caption{Overview of the proposed method, UNICORN, for unified conversational recommendation policy learning. Shallowed and opaqued nodes represent accepted and rejected actions, respectively.}
\label{method}
\vspace{-0.3cm}
\end{figure*}

The overview of the proposed method, UNICORN, is depicted in Figure~\ref{method}, which consists of four main components: Graph-based MDP Environment, State Representation Learning, Action Selection Strategy, and Deep Q-Learning Network.  


\subsection{Graph-based MDP Environment}
The MDP environment is responsible for informing the agent about the current state and possible actions to take, and then rewards the agent based on how the current policy fits the observed user interactions. Formally, the MDP environment can be defined by a tuple $(\mathcal{S},\mathcal{A},\mathcal{T},\mathcal{R})$, where $\mathcal{S}$ denotes the state space, $\mathcal{A}$ denotes the action space, $\mathcal{T}:\mathcal{S}\times\mathcal{A}\rightarrow \mathcal{S}$ refers to the state transition function, and $\mathcal{R}:\mathcal{S}\times\mathcal{A}\rightarrow \mathbb{R}$ is the reward function. 

\subsubsection{\textbf{State}}
As for the graph-based MDP environment, the state $s_t\in\mathcal{S}$ at timestep $t$ is supposed to contain all the given information for conversational recommendation, including the previous conversation history and the full graph $\mathcal{G}$ that contains all the users, items, and attributes. 
Given a user $u$, we consider two major elements:
\begin{equation}
    s_t = [\mathcal{H}_u^{(t)},\mathcal{G}_u^{(t)}],
\end{equation}
where $\mathcal{H}_u^{(t)} = [\mathcal{P}_u^{(t)}, \mathcal{P}_{\mathrm{rej}}^{(t)}, \mathcal{V}_{\mathrm{rej}}^{(t)}]$ denotes the conversation history until timestep $t$, and $\mathcal{G}_u^{(t)}$ denotes the dynamic subgraph of $\mathcal{G}$ for the user $u$ at  timestep $t$ (The graph construction will be introduced in Section~\ref{sec:state}). $\mathcal{P}_u$ denotes the user-preferred attribute. $\mathcal{P}_{\mathrm{rej}}$ and $\mathcal{V}_{\mathrm{rej}}$ are the attributes and items rejected by the user, respectively.
The initial state $s_0$ is initialized by the user specifying an attribute $p_0$, i.e., $s_0 = [[\{p_0\},\{\},\{\}],\mathcal{G}_u^{(0)}]$.

\subsubsection{\textbf{Action}}
According to state $s_t$, the agent takes an action $a_t\in\mathcal{A}$, where $a_t$ can be selected from the candidate item set $\mathcal{V}_{\mathrm{cand}}^{(t)}$ to recommend items or from the candidate attribute set $\mathcal{P}_{\mathrm{cand}}^{(t)}$ to ask attributes. Following the path reasoning approach~\cite{kdd20-scpr}, we have
\begin{align}
    \mathcal{V}_{\mathrm{cand}}^{(t)} = \mathcal{V}_{\mathcal{P}_u^{(t)}}\setminus \mathcal{V}_{\mathrm{rej}}^{(t)},\quad
    \mathcal{P}_{\mathrm{cand}}^{(t)} = \mathcal{P}_{\scaleto{\mathcal{V}_{\mathrm{cand}}^{(t)}}{9pt}  }\setminus(\mathcal{P}_u^{(t)}\cup\mathcal{P}_{\mathrm{rej}}^{(t)}),
\end{align}
where $\mathcal{V}_{\mathcal{P}_u^{(t)}}$ is the set of item vertices directly connecting all $\mathcal{P}_u^{(t)}$ (i.e., items satisfying all the preferred attributes), and $\mathcal{P}_{\scaleto{\mathcal{V}_{\mathrm{cand}}^{(t)}}{9pt}}$ is the set of attribute vertices directly connecting to one of $\mathcal{V}_{\mathrm{cand}}^{(t)}$ (i.e., attributes belonging to at least one of the candidate items).

\subsubsection{\textbf{Transition}}
We consider that current state $s_t$ will transition to the next state $s_{t+1}$ when the user responds to the action $a_t$. In specific, if CRS asks an attribute $p_t$ and the user accepts it, the next state $s_{t+1}$ will be updated by $\mathcal{P}_u^{(t+1)}=\mathcal{P}_u^{(t)}\cup p_t$. Conversely, if the user rejects the action $a_t$, $s_{t+1}$ will be updated by $\mathcal{P}_{\mathrm{rej}}^{(t+1)}=\mathcal{P}_{\mathrm{rej}}^{(t)}\cup a_t$ or $\mathcal{V}_{\mathrm{rej}}^{(t+1)}=\mathcal{V}_{\mathrm{rej}}^{(t)}\cup a_t$ for $a_t\in\mathcal{P}$ and $a_t\in\mathcal{V}$, respectively. As a result, the next state $s_{t+1}$ will be $[\mathcal{H}_u^{(t+1)},\mathcal{G}_u^{(t+1)}]$.


\subsubsection{\textbf{Reward}} 
Following previous MCR studies~\cite{wsdm20-ear,kdd20-scpr}, our environment contains five kinds of rewards, namely, (1) $r_{\mathrm{rec\_suc}}$, a strongly positive reward when the user accepts the recommended items,  (2) $r_{\mathrm{rec\_fail}}$, a negative reward when the user rejects the recommended items, (3) $r_{\mathrm{ask\_suc}}$, a slightly positive reward when the user accepts the asked attribute, (4) $r_{\mathrm{ask\_fail}}$, a negative reward when the user reject the asked attribute, and (5) $r_{\mathrm{quit}}$, a strongly negative reward when reaching the maximum number of turns.


\subsection{Graph-enhanced State Representation}
\label{sec:state}

As we formulate conversational recommendation as a unified policy problem over a graph-based MDP environment, it is required to encode both the conversational and structural information into the latent distributed representations. In order to make use of the interrelationships among users, items, and attributes, we first adopt graph-based pre-training methods~\cite{transe,transh} to obtained node embeddings for all the nodes in the full graph $\mathcal{G}$.

\subsubsection{\textbf{Dynamic Weighted Graph Construction}}
During the conversation, we represent the current state of the graph-based MDP environment as a dynamic weighted graph.
Formally, we denote an undirected weighted graph as $\mathcal{G}=(\mathcal{N},\bm{A})$, with nodes $n_i\in\mathcal{N}$, the adjacency matrix $\bm{A}_{i,j}$ that denotes the weighted edges between nodes $n_i$ and $n_j$. In our case, given the user $u$, we denote the dynamic graph at timestep $t$ as $\mathcal{G}_u^{(t)}=(\mathcal{N}^{(t)},\bm{A}^{(t)})$:
\begin{equation}
    \mathcal{N}^{(t)} = \{u\}\cup\mathcal{P}_u^{(t)}\cup\mathcal{P}_{\mathrm{cand}}^{(t)}\cup\mathcal{V}_{\mathrm{cand}}^{(t)},
\end{equation}
\begin{equation}
    \bm{A}^{(t)}_{i,j} =
  \begin{cases}
    w_v^{(t)},     & \quad \text{if } n_i = u, n_j \in \mathcal{V} \\
    1,       & \quad \text{if } n_i \in \mathcal{V}, n_j \in \mathcal{P} \\
    0,       & \quad \text{otherwise}
  \end{cases} 
\label{eq:a}
\end{equation}
where $w_v^{(t)}$ is a scalar indicating the recommendation score of item $v$ in the current state. In order to incorporate the user preference as well as the correlation between the asked attributes and the items, this weight $w_v^{(t)}$ is calculated by
\begin{equation}
    w_v^{(t)} = \sigma\Bigl(e_u^\top e_v + \sum\nolimits_{\scaleto{p\in\mathcal{P}_u^{(t)}}{8pt}} e_v^\top e_p - \sum\nolimits_{\scaleto{p\in\mathcal{P}_{\mathrm{rej}}^{(t)}\cap\mathcal{P}_v^{(t)}}{8pt}} e_v^\top e_p\Bigr),
\label{item_weight}
\end{equation}
where $\sigma(\cdot)$ denotes the sigmoid function, $e_u$, $e_v$, and $e_p$ are the embeddings of corresponding users, items, and attributes, respectively. 

\subsubsection{\textbf{Graph-based Representation Learning}}
In order to comprehensively take advantage of the correlation information among the user, items, and attributes from the connectivity in the graph, we employ a graph convolutional network (GCN)~\cite{iclr17-gcn} to refine the node representations with structural and relational knowledge. The representations of node $n_i$ in $(l+1)$-th layer can be computed by:
\begin{equation}
    e_i^{(l+1)} = \text{ReLU}\left(\sum\nolimits_{j\in \mathcal{N}_i}\bm{\Lambda}_{i,j}\bm{W}_{l}e_j^{(l)} + \bm{B}_le_i^{(l)}\right),
\end{equation}
where $\mathcal{N}_i$ denotes the neighboring indices of the node $n_i$, $\bm{W}_{l}$ and $\bm{B}_{l}$ are trainable parameters representing the transformation from neighboring nodes and the node $n_i$ itself, and $\bm{\Lambda}$ is a normalization adjacent matrix as $\bm{\Lambda} = \bm{D}^{-\frac{1}{2}}\bm{A}\bm{D}^{-\frac{1}{2}}$ with $\bm{D}_{ii} =\sum_j \bm{A}_{i,j} $..

\subsubsection{\textbf{Sequential Representation Learning}}
Apart from the interrelationships among the user, items, and attributes, the CRS are also expected to model the conversation history in current state. Unlike previous studies~\cite{wsdm20-ear,kdd20-scpr} which adopt heuristic features for conversation history modeling, we employ Transformer encoder~\cite{transformer} for capturing the sequential information of the conversation history as well as attending the important information for deciding the next action. As described in \cite{transformer}, each transformer layer consists of three components: (i) The layer normalization is defined as LayerNorm$(\cdot)$. (ii) The multi-head attention is defined as MultiHead$(\bm{Q}, \bm{K}, \bm{V})$, where $\bm{Q}, \bm{K}, \bm{V}$ are query, key, and value, respectively. (iii) The feed-forward network with ReLU activation is defined as FFN$(\cdot)$. Take the $l$-th layer for example: 
\begin{align}
    \bm{X}^* &= \text{MultiHead}(\bm{X}^{(l)},\bm{X}^{(l)},\bm{X}^{(l)}), \\
    \bm{X}^{(l+1)} &=\text{LayerNorm}(\text{FFN}(\bm{X}^*) + \bm{X}^{(l)}),
\end{align}
where $\bm{X}\in\mathbb{R}^{L\times d}$ denotes their embeddings, and $L$ is the sequence length. 
In our case, the input sequence $\bm{X}^{(0)}$ is the accepted attributes $\mathcal{P}_u^{(t)}$ in current conversation history with the learned graph-based representation $\{e_p^{(L_g)}:p\in\mathcal{P}_u^{(t)}\}$, where $L_g$ is the number of layers in GCN. After the sequential learning with $L_s$ transformer layers, we can aggregate the information learned from both the graph and the conversation history by a mean pooling layer to obtain the state representation of $s_t$:
\begin{equation}
    f_{\theta_S}(s_t) = \text{MeanPool}(\bm{X}^{L_s}).
\label{state_rep}
\end{equation}
For simplicity, we denote the learned state representation of $s_t$ as $f_{\theta_S}(s_t)$, where $\theta_S$ is the set of the whole network parameters for state representation learning, including parameters of GCN and Transformer layers. 


\subsection{Action Selection Strategy}
\label{sec:action}
A large action search space will harm the performance of the policy learning to a great extent~\cite{kdd20-scpr}. Thus, it attaches great importance to handle the overwhelmingly large action space in UCRPL.
To this end, we propose two simple strategy to improve the sample efficiency for candidate action selection. 

\noindent \textbf{Preference-based Item Selection}. In general, as for candidate items to be recommended, since users are not likely to be interested in all items, we can only consider the action of making recommendations from a small amount of candidate items that fit the user preference the most. To achieve this, we select top-$K_v$ candidate items from $\mathcal{V}_{\mathrm{cand}}^{(t)}$ into the candidate action space $\mathcal{A}_t$ at each timestep $t$, where the candidate items is ranked by the recommendation score $w_v$ in Equation~\ref{item_weight}.  

\noindent \textbf{Weighted Entropy-based Attribute Selection}. Whereas for candidate attributes to be asked, the expected one is supposed to be able to not only better eliminate the uncertainty of candidate items, but also encode the user preference. Inspired by~\cite{kdd20-scpr}, we adopt weighted entropy as the criteria to prune candidate attributes:
\begin{align}
    w_p &= - \text{prob}(p)\cdot\log(\text{prob}(p)),\\
    \text{prob}(p) &= \sum\nolimits_{v\in\mathcal{V}_{\mathrm{cand}}\cap\mathcal{V}_p}w_v \Big/ \sum\nolimits_{v\in\mathcal{V}_{\mathrm{cand}}}w_v,
\end{align}
where $w_p$ is the weighted entropy score for attribute $p$, and $\mathcal{V}_p$ denotes the items that include the attribute $p$. Similar to item selection, we also select top-$K_p$ candidate attributes from $\mathcal{P}_{\mathrm{cand}}^{(t)}$ into $\mathcal{A}_t$ based on $w_p$. 


\begin{algorithm}[t]
\small
\caption{Unified Conversational Recommender}
\label{algo}
\KwIn{$\{\mathbf{e}_i\}_{i\in \mathcal{N}}$; $\mathcal{D}$;  $\tau$; $\epsilon$; $\gamma$; $K$; $T$; $K_v$; $K_p$;} 
\KwOut{ $\theta_S$;  $\theta_Q$; }
Initialize all parameters: $\theta_S$, $\theta_Q$, $\theta_Q' \leftarrow \theta_Q$\;

\For{$\mathit{episode} = 1, 2, \ldots , N$}{

User $u$ starts the conversation by specifying an attribute $p_0$\;

Update: $\mathcal{P}_u^{(0)} = \{p_0\}$, $\mathcal{P}_{\mathrm{rej}}^{(0)}=\{\}$, $\mathcal{V}_{\mathrm{rej}}^{(0)}=\{\}$, $\mathcal{H}_u^{(0)} = [\mathcal{P}_u^{(0)},\mathcal{P}_{\mathrm{rej}}^{(0)},\mathcal{V}_{\mathrm{rej}}^{(0)}]$, $s_0 = [\mathcal{H}_u^{(0)}, \mathcal{G}_u^{(0)}]$\;
Get candidate action space $\mathcal{A}_0$ via Action Selection\;
		
\For{turn $t = 0, 1, \ldots , T-1$}{
	
	Get state representation $f_{\theta_S}(s_t)$ via Eq.(\ref{state_rep})\;
	Select an action $a_t$ by $\epsilon$-greedy w.r.t Eq.(\ref{q-value})\;%$\argmax_{a_t\in\mathcal{A}_t}Q(s_t,a_t)$
	
	Receive reward $r_t$\;
	Update the next state $s_{t+1} = \mathcal{T}(s_t,a_t)$\;
	Get $\mathcal{A}_{t+1}$ via Action Selection\;
	Store $(s_t, a_t, r_t, s_{t+1}, \mathcal{A}_{t+1})$ to buffer $\mathcal{D}$\;
	Sample mini-batch of $(s_t, a_t, r_t, s_{t+1}, \mathcal{A}_{t+1})$ w.r.t Eq.(\ref{per})\;
	Compute the target value $y_t$ via Eq.~(\ref{target_value})\;
	Update $\theta_S$, $\theta_Q$ via SGD w.r.t the loss function Eq.(\ref{loss})\;
	Update $\theta_Q'$ via Eq.(\ref{double}) \;
}
}
\end{algorithm}
\setlength{\textfloatsep}{0pt}


\subsection{Deep Q-Learning Network}
After obtaining the graph-enhanced state representation and the candidate action space, we introduce the deep Q-learning network (DQN)~\cite{nature-dqn} to conduct the unified conversational recommendation policy learning. We further implement three techniques to enhance and stabilize the training of DQN, including double Q-learning~\cite{aaai16-doubledqn}, prioritized replay~\cite{iclr16-per}, and dueling network~\cite{icml16-dueling}. The training procedure of the proposed Unified Conversational Recommendation Policy Learning is presented in Algorithm~\ref{algo}.


\subsubsection{\textbf{Dueling Q-Network}}
Following the standard assumption that delayed rewards are discounted by a factor of $\gamma$ per timestep, we define
the Q-value $Q(s_t, a_t)$ as the expected reward based on state $s_t$ and action $a_t$. 
As shown in the rightmost part of Figure~\ref{method}, the dueling Q-network~\cite{icml16-dueling} employs two deep neural networks to compute the value function $V(a_t)$ and advantage function $A(f_{\theta_S}(s_t), a_t)$, respectively. Then the Q-function can be calculated by:
\begin{equation}\label{q-value}
    Q(s_t, a_t) = V(a_t) + A(f_{\theta_S}(s_t), a_t),
\end{equation}
where $V(\cdot)$ and $A(\cdot)$ are two separate multi-layer perceptions with parameters denoted as $\theta_V$ and $\theta_A$ respectively, and let $\theta_Q = \{\theta_V, \theta_A\}$.

The optimal Q-function $Q^*(s_t, a_t)$, which has the maximum expected reward achievable by the optimal policy $\pi^*$, follows the Bellman equation~\cite{bellman} as:
\begin{equation}
    Q^*(s_t, a_t) = \mathbb{E}_{s_{t+1}}\Bigl[r_t+\gamma \max_{a_{t+1}\in\mathcal{A}_{t+1}}\! Q^*(s_{t+1},a_{t+1})|s_t,a_t\Bigr].
\end{equation}



\subsubsection{\textbf{Double Q-Learning with Prioritized Experience Replay}}
During each episode in the MCR process, at each timestep $t$, the CRS agent obtains the current state representation $f_{\theta_S}(s_t)$ via the graph-enhanced state representational learning described in Section~\ref{sec:state}. Then the agent selects an action $a_t$ from the candidate action space $\mathcal{A}_t$, which is obtained via the action selection strategies described in Section~\ref{sec:action}. Here we incorporate $\epsilon$-greedy method for balance the exploration and exploitation in action sampling (i.e., select a greedy action based on the max Q-value with probability $1-\epsilon$, and a random action with probability $\epsilon$).

Then, the agent will receive the reward $r_t$ from the user's feedback. According to the feedback, the current state $s_t$ transitions to the next state $s_{t+1}$, and the candidate action space $\mathcal{A}_{t+1}$ is updated correspondingly. The experience $(s_t, a_t, r_t, s_{t+1}, \mathcal{A}_{t+1})$ is then stored into the replay buffer $\mathcal{D}$. To train DQN, we sample mini-batch of experiences from $\mathcal{D}$, and minimize the following loss function:
\begin{align}
    \mathcal{L}(\theta_Q, \theta_S) &= \mathbb{E}_{(s_t,a_t,r_t,s_{t+1},\mathcal{A}_{t+1}){\sim}\mathcal{D}}\bigl[(y_t {-} Q(s_t,a_t;\theta_Q,\theta_S))^2\bigr], \label{loss}\\
    y_t &= r_t + \gamma \max_{a_{t+1}\in\mathcal{A}_{t+1}} Q(s_{t+1},a_{t+1};\theta_Q,\theta_S). \label{eq:yt}
\end{align}
where $y_t$ is the target value based on the currently optimal $Q^*$. 

To alleviate the overestimation bias problem in conventional DQN, we adopt Double Q-learning~\cite{aaai16-doubledqn}, which employs a target network $Q'$ as a copy from the online network but updated with certain training delay. The target value of the online network is then changed to:
\begin{equation}
    y_t = r_t + \gamma Q'\bigl(s_{t+1}, \argmax_{a_{t+1}\in\mathcal{A}_{t+1}} Q(s_{t+1},a_{t+1};\theta_Q,\theta_S);\theta_{Q'},\theta_S\bigr),
\label{target_value}
\end{equation}
where $\theta_{Q'}$ denotes the parameter of the target network, which is updated by the soft assign as:
\begin{equation}
    \theta_{Q'} = \tau\theta_{Q} + (1-\tau)\theta_{Q'}
\label{double}
\end{equation}
where $\tau$ is the update frequency.

In addition, conventional DQN samples uniformly from the replay buffer. In order to sample more frequently those important transitions from which there is much to learn. As a proxy for learning potential, prioritized replay~\cite{iclr16-per} samples transitions with probability $\delta$ relative to the last encountered absolute TD error:
\begin{equation}
    \delta \propto \Bigl|r_{t+1} + \gamma Q'\bigl(s_{t+1},\argmax_{a_{t+1}\in\mathcal{A}_{t+1}} Q(s_{t+1},a_{t+1})\bigr) - Q(s_t,a_t)\Bigr|.
\label{per}
\end{equation}

\subsubsection{\textbf{Model Inference}}
With the learned UNICORN model, given a user and his/her conversation history, we follow the same process to obtain the candidate action space and the current state representation, and then decide the next action according to max Q-value in Eq.(\ref{q-value}). 
If the selected action points to an attribute, the system will ask the user's preference on the attribute. Otherwise, the system will recommend top-$K$ items with the highest Q-value to the user.







\section{Experiment}


\subsection{Dataset}
We evaluate the proposed method on four existing multi-round conversational recommendation benchmark datasets and further construct a new dataset from real-world E-Commerce platform. The statistics of these datasets are presented in Table~\ref{dataset} and the corresponding descriptions are as follows.

\begin{itemize}[leftmargin=*,topsep=4pt]
    \item \textbf{LastFM} and \textbf{Yelp}. The LastFM dataset is used for evaluation on music artist recommendation, while the Yelp dataset is for business recommendation. \citet{wsdm20-ear} manually categorize the original attributes in LastFM into 33 coarse-grained groups, and build a 2-layer taxonomy with 29 first-layer categories for Yelp. 
    \item \textbf{LastFM*} and \textbf{Yelp*}. \citet{kdd20-scpr} consider the manual efforts to merge attributes are not realistic for practical applications, so they adopt original attributes to reconstruct these two datasets.
    \item \textbf{E-Commerce}. In order to evaluate the proposed method in real-world E-Commerce scenario, we collect the dataset by sampling logs from a well-known E-Commerce platform in the same way as LastFM and Yelp. We randomly sample 30,000 items from the Women\_Dress category and a certain number of users who have interacted with these items. And we treat the concatenation of the product property and the property value as the attribute to be asked, e.g., ``Color=Red", where ``Color" is a product property and ``Red" is a property value. Following the MCR data construction described in \citet{wsdm20-ear}, we obtain the E-Commerce dataset with the statistics shown in Table~\ref{dataset}. As for the graph construction, we only consider two kinds of relations, including ``purchased\_by (item$\rightarrow$ user)" and ``belong\_to (attribute$\rightarrow$ item)" for simplification. Compared with the imbalanced ratio of \#items:\#attributes at LastFM (0.88:1) and Yelp (119:1), the E-Commerce dataset preserves a large number of items as well as attributes, which is more in line with the real-world applications in E-Commerce. 
\end{itemize}

\begin{table}
\setlength{\abovecaptionskip}{2pt}   
\setlength{\belowcaptionskip}{2pt}
\centering
  \caption{Summary statistics of datasets.}
\begin{adjustbox}{max width=\linewidth}
\setlength{\tabcolsep}{1mm}{
\begin{tabular}{lrrrrr}
\toprule 
& LastFM & LastFM $^{*}$ & Yelp & Yelp* & E-Comm \\
\midrule 
 \#Users & 1,801 & 1,801 & 27,675 & 27,675 & 26,430 \\
 \#Items & 7,432 & 7,432 & 70,311 & 70,311 & 29,428 \\
 \#Interactions & 76,693 & 76,693 & 1,368,606 & 1,368,606 & 748,533 \\
 \#Attributes & 33 & 8,438 & 29 & 590 & 1,413 \\
\midrule 
\#Entities & 9,266 & 17,671 & 98,605 & 98,576 & 57,271 \\
 \#Relations & 4 & 4 & 3 & 3 & 2 \\
 \#Triplets & 138,215 & 228,217 & 2,884,567 & 2,533,827 & 2,024,962 \\
\bottomrule
\label{dataset}
\end{tabular}}
\end{adjustbox}
\vspace{-0.3cm}
\end{table}

\begin{table*}
\setlength{\abovecaptionskip}{2pt}   
\setlength{\belowcaptionskip}{2pt}
\centering
  \caption{Experimental Results. $^\dagger$ indicates statistically significant improvement ($p<0.01$) over all baselines. hDCG stands for hDCG@(15,10). The SR@15 and AT scores of baseline methods on the first four datasets are derived from \citet{kdd20-scpr}.}
\begin{adjustbox}{max width=\textwidth}
\setlength{\tabcolsep}{1mm}{
\begin{tabular}{lccccccccccccccc}
\toprule 
& \multicolumn{3}{c} { LastFM } & \multicolumn{3}{c} { LastFM*} & \multicolumn{3}{c} { Yelp} & \multicolumn{3}{c} { Yelp* } & \multicolumn{3}{c} { E-Commerce}\\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16}
& SR@15 & AT &hDCG & SR@15 & AT&hDCG & SR@15 & AT&hDCG & SR@15 & AT&hDCG& SR@15 & AT &hDCG\\
\midrule 
Abs Greedy & 0.222 & 13.48 &0.073& 0.635 & 8.66 &0.267& 0.264 & 12.57 &0.145& 0.189 & 13.43 &0.089& 0.273&12.19&0.138 \\
Max Entropy & 0.283 & 13.91 &0.083& 0.669 & 9.33 &0.269& 0.921 & 6.59 &0.338& 0.398 & 13.42&0.121&0.328&12.98& 0.112\\
CRM~\cite{sigir18-crm} & 0.325 & 13.75 &0.092& 0.580 & 10.79 &0.224& 0.923 & 6.25 &0.353& 0.177 & 13.69&0.070&0.294&12.11&0.146 \\
EAR~\cite{wsdm20-ear} & 0.429 & 12.88 &0.136& 0.595 & 10.51 &0.230& 0.967 & 5.74 &0.378& 0.182 & 13.63 &0.079&0.381&\underline{11.48}&0.161\\
SCPR~\cite{kdd20-scpr} & $\underline{0.465}$ & $\underline{12.86}$ & \underline{0.139} &$\underline{0.709}$ & $\underline{8.43}$ & 0.317 &$\underline{0.973}$ & $\underline{5.67}$ & \underline{0.382} &$\underline{0.489}$ & $\underline{12.62}$ &0.159 &\underline{0.518} &12.32&\underline{0.168}\\
\midrule 
\textbf{UNICORN} & $\mathbf{0.535}$$^\dagger$ & $\mathbf{11.82}$$^\dagger$ &\textbf{0.175}$^\dagger$& $\mathbf{0 . 788}$$^\dagger$ & $\mathbf{7 . 58}$$^\dagger$ &\textbf{0.349}$^\dagger$& $\mathbf{0 . 9 8 5}$$^\dagger$ & $\mathbf{5 . 33}$$^\dagger$ &\textbf{0.397}$^\dagger$& $\mathbf{0 . 520}$$^\dagger$ & $\mathbf{11 .31}$$^\dagger$&\textbf{0.203}$^\dagger$&\textbf{0.602$^\dagger$}&\textbf{10.45}$^\dagger$ &\textbf{0.217}$^\dagger$\\
\bottomrule
\label{result}
\end{tabular}}
\end{adjustbox}
\vspace{-0.5cm}
\end{table*}

\iffalse
\begin{table*}
\setlength{\abovecaptionskip}{2pt}   
\setlength{\belowcaptionskip}{2pt}
\centering
  \caption{Experimental Results. $^\dagger$ indicates statistically significant improvement ($p<0.01$) over all baselines.}
\begin{tabular}{lcccccccccc}
\toprule 
& \multicolumn{2}{c} { LastFM } & \multicolumn{2}{c} { LastFM*} & \multicolumn{2}{c} { Yelp} & \multicolumn{2}{c} { Yelp* } & \multicolumn{2}{c} { E-Commerce}\\
\cmidrule{2-11}
& SR@15 & AT & SR@15 & AT & SR@15 & AT & SR@15 & AT& SR@15 & AT \\
\midrule 
Abs Greedy & 0.222 & 13.48 & 0.635 & 8.66 & 0.264 & 12.57 & 0.189 & 13.43 & 0.273&12.19 \\
Max Entropy & 0.283 & 13.91 & 0.669 & 9.33 & 0.921 & 6.59 & 0.398 & 13.42&0.328&12.98 \\
CRM~\cite{sigir18-crm} & 0.325 & 13.75 & 0.580 & 10.79 & 0.923 & 6.25 & 0.177 & 13.69&0.294&12.11 \\
EAR~\cite{wsdm20-ear} & 0.429 & 12.88 & 0.595 & 10.51 & 0.967 & 5.74 & 0.182 & 13.63 &0.381&11.48\\
SCPR~\cite{kdd20-scpr} & $\underline{0.465}$ & $\underline{12.86}$ & $\underline{0.709}$ & $\underline{8.43}$ & $\underline{0.973}$ & $\underline{5.67}$ & $\underline{0.489}$ & $\underline{12.62}$ & \underline{0.518} &\underline{12.32}\\
\midrule 
\midrule
\textbf{UNICORN} & \textbf{0.535}$^\dagger$ & \textbf{11.82}$^\dagger$ & \textbf{0.788}$^\dagger$ & \textbf{7 . 58}$^\dagger$ & \textbf{0.985}$^\dagger$ & \textbf{5.33}$^\dagger$ & \textbf{0.520}$^\dagger$ & \textbf{11.31}$^\dagger$&\textbf{0.602$^\dagger$}&\textbf{10.45}$^\dagger$ \\
\bottomrule
\end{tabular}
\label{result}
\end{table*}
\fi

\subsection{Experimental Settings}
\subsubsection{\textbf{User Simulator}}\label{sec:user_sim} 
Due to the interactive nature of MCR, it needs to be trained and evaluated by interacting with users. Following the user simulator adopted in~\cite{sigir18-crm,wsdm20-ear}, we simulate a conversation session for each observed user-item interaction pair $(u,v)$. We regard the item $v$ as the ground-truth target item and treat its attribute set $\mathcal{P}_v$ as the oracle set of attributes preferred by the user $u$ in this conversation session. The session is initialized by the simulated user to specify a certain attribute, which is randomly chosen from $\mathcal{P}_v$. Then the session follows the process of ``System Ask, User Respond"~\cite{cikm18-saur} as introduced in Section~\ref{sec:method}. 

\subsubsection{\textbf{Baselines}}
We compare the proposed method with several state-of-the-art methods on MCR as follows:
\begin{itemize}[leftmargin=*,topsep=4pt]
    \item \textbf{Max Entropy}. This is a rule-based strategy to decide the next action, where the CRS selects an attribute to ask based on the maximum entropy within the current state and chooses to recommend the top ranked items with a certain probability~\cite{wsdm20-ear}.
    \item \textbf{Abs Greedy}~\cite{kdd16-convbandit}. This method only performs recommendation actions and updates itself until the CRS makes successful recommendation or exceed the maximum turns of conversation.
    \item \textbf{CRM}~\cite{sigir18-crm}. This method is originally designed for single-round conversational recommendation, which employs policy gradient~\cite{nips99-pg} to learn the policy deciding when and which attributes to ask. We follow~\cite{wsdm20-ear} for the adaptation into MCR scenario.
    \item \textbf{EAR}~\cite{wsdm20-ear}. A three-stage method is proposed to enhance the interaction between the conversation and recommendation components with a similar RL framework as CRM.
    \item \textbf{SCPR}~\cite{kdd20-scpr}. This is the state-of-the-art method on MCR setting, which leverages interactive path reasoning on the graph to prune off candidate attributes and adopts the DQN~\cite{nature-dqn} framework to determine when to ask or recommend.
\end{itemize}

\subsubsection{\textbf{Evaluation Metrics}}
Following previous studies on multi-round conversational recommendation~\cite{wsdm20-ear,kdd20-scpr}, we adopt success rate at turn $t$ (SR@$t$)~\cite{sigir18-crm} to measure the cumulative ratio of successful conversational recommendation by turn $t$. Besides, average turn (AT) is adopted to evaluate the average number of turns for all sessions (if the conversation session reaches the maximum turn $T$, the turn for such session is also counted by $T$). To be specific, the higher SR@$t$ indicates a better performance of the CRS at a turn $t$, while the lower AT means an overall higher efficiency of the CRS. 

Although SR@$t$ and AT are widely adopted for the evaluation of CRS, both of them are not sensitive to the rank order in the recommendation results and only consider a certain aspect of the performance of CRS. 
In order to conduct a comprehensive evaluation of CRS, we propose to extend the normalized discounted cumulative gain (NDCG@$K$) to be a two-level hierarchical version, namely \textbf{hNDCG@($\bm{T,K}$)}, with the definition as follows:
\begin{equation}
    \begin{aligned}
    hDCG@(T,K) =& \sum\nolimits_t^T\sum\nolimits_k^Kr(t,k)\left[\frac{1}{\log_2(t+2)}\right.\\
    &\left. +\left(\frac{1}{\log_2(t{+}1)}-\frac{1}{\log_2(t{+}2)}\right)\frac{1}{\log_2(k{+}1)} \right],
\end{aligned}
\end{equation}
where $T$ and $K$ represent the number of conversation turns and recommended items in each turn, $r(t,k)$ denotes the relevance of the result at turn $t$ and position $k$.
Then hNDCG@($T,K$) can be drawn from hDCG@($T,K$) with the same way as the original NDCG@$K$. And since there is only one target item for each interaction in our case, we simply use hDCG@($T,K$) for evaluation. The intuition behind hNDCG@($T,K$) is that the less turn of a successful session is the prior interest for the CRS, while the target item is expected to be ranked higher in the recommendation list at the success turn. 




\subsubsection{\textbf{Implementation Details}}
Following the data split in~\cite{kdd20-scpr}, we also split the E-Commerce dataset by 7:1.5:1.5 for training, validation, and testing. And set the size $K$ of the recommendation list as 10, and maximum turn $T$ as 15. 
%Different from existing methods for MCR~\cite{wsdm20-ear,sigir18-crm,kdd20-scpr}, which requires to train an offline recommendation models (e.g., FM) as well as pretrain the policy network with offline dialogue history, we can simply initialize the whole framework with pretrained graph-based embeddings. 
We adopt TransE~\cite{transe} from OpenKE~\cite{openke} to pretrain the node embeddings in the constructed graph with the training set. 
We use the user simulator described in Section~\ref{sec:user_sim} to interact with the proposed CRS for online training the model using the validation set.  For all implemented methods, we conduct the online training for 10,000 episodes. To maintain a fair comparison with other baselines~\cite{wsdm20-ear,kdd20-scpr}, we adopt the same reward settings to train the proposed model: $r_{\mathrm{rec\_suc}}$=1, $r_{\mathrm{rec\_fail}}$=-0.1, $r_{\mathrm{ask\_suc}}$=0.01, $r_{\mathrm{ask\_fail}}$=-0.1, $r_{\mathrm{quit}}$=-0.3. The hyper-parameters are empirically set as follows: The embedding size and the hidden size are set to be 64 and 100. The number of GCN layers $L_g$ and Transformer layers $L_s$ is set to be 2 and 1, respectively. The number of selected candidate attributes $K_p$ and items $K_v$ is set to be 10. 
%Here we use the same hyper-parameter setting across different datasets for simplification. More details can be found in the following sections. 
During the training procedure of DQN, the size of experience replay buffer is 50,000, and the size of mini-batch is 128. The learning rate and the $L_2$ norm regularization are set to be 1e-4 and 1e-6, with Adam optimizer. The discount factor $\gamma$ and the update frequency $\tau$ are set to be 0.999 and 0.01. 


\begin{figure}
\setlength{\abovecaptionskip}{2pt}   
\setlength{\belowcaptionskip}{2pt}
\centering
\includegraphics[width=0.48\textwidth]{exp1.pdf}
\caption{Comparisons at Different Conversation Turns.}
\label{diff_turn}
\vspace{0.1cm}
\end{figure}


\subsection{Performance Comparison}
\subsubsection{\textbf{Overall Performance}}

\begin{table*}
\setlength{\abovecaptionskip}{2pt}   
\setlength{\belowcaptionskip}{2pt}
\centering
  \caption{Ablation Study. }
\begin{adjustbox}{max width=\textwidth}
\setlength{\tabcolsep}{1mm}{
\begin{tabular}{lccccccccccccccc}
\toprule 
& \multicolumn{3}{c} { LastFM } & \multicolumn{3}{c} { LastFM*} & \multicolumn{3}{c} { Yelp} & \multicolumn{3}{c} { Yelp* } & \multicolumn{3}{c} { E-Commerce}\\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16}
& SR@15 & AT &hDCG & SR@15 & AT &hDCG & SR@15 & AT &hDCG & SR@15 & AT &hDCG& SR@15 & AT &hDCG\\
\midrule 
\textbf{UNICORN} & 0.535 & \textbf{11.82} &\textbf{0.175}& \textbf{0.788} & \textbf{7.58} &\textbf{0.349}& \textbf{0.985} & \textbf{5.33} &0.397& \textbf{0.520} & \textbf{11.31}&\textbf{0.203}&\textbf{0.602}&\textbf{10.45} &\textbf{0.217}\\
\midrule
(a) - RNN &\textbf{0.539}&11.85&0.173&0.763&7.59&0.341&0.980&5.36&\textbf{0.401}&0.509&11.25&0.189&0.588&10.84&0.208\\
(b) - w/o Transformer&0.478&12.17&0.147&0.733&7.78&0.320&0.958&6.18&0.370&0.470&11.62&0.167&0.545&11.23&0.178\\
(c) - w/o GCN&0.440&12.74&0.139&0.744&7.62&0.327&0.978&5.48&0.394&0.481&11.45&0.171&0.554&11.07&0.183\\
\midrule
(d) - Random Embeddings&0.310&13.31&0.096&0.665&9.24&0.291&0.905&7.66&0.318&0.196&13.95&0.049&0.220&13.55&0.069\\
(e) - FM Embeddings&0.465 & 12.26&0.144 & 0.748 & 7.68&0.328 & 0.982 &5.50& 0.394& 0.496 & 12.25&0.161&0.579&10.89&0.202\\
\midrule 
(f) - Preference-based Attr. Sel.&0.467&12.33&0.129&0.712&8.24&0.303&0.978&5.74&0.385&0.489&11.60&0.171&0.569&11.06&0.206\\
(g) - Entropy-based Attr. Sel.&0.507&11.96&0.165&0.756&7.63&0.324&0.978&5.71&0.388&0.502&11.33&0.192&0.585&10.69&0.214\\
(h) - w/o Attribute Selection&0.487&12.12&0.151&0.604&9.88&0.258&0.942&6.80&0.357&0.220&12.97&0.067&0.434&12.01&0.127\\
(i) - w/o Item Selection&0.150&13.83&0.055&0.638&8.85&0.294&0.780&9.16&0.276&0.158&13.60&0.054&0.144&13.85&0.056\\
\bottomrule
\end{tabular}}
\end{adjustbox}
\label{ablation}
\vspace{-0.3cm}
\end{table*}

\iffalse
\begin{table*}
\setlength{\abovecaptionskip}{2pt}   
\setlength{\belowcaptionskip}{2pt}
\centering
  \caption{Ablation Study.}
\begin{tabular}{lcccccccccc}
\toprule 
& \multicolumn{2}{c} { LastFM } & \multicolumn{2}{c} { LastFM*} & \multicolumn{2}{c} { Yelp} & \multicolumn{2}{c} { Yelp* } & \multicolumn{2}{c} { E-Commerce}\\
\cmidrule{2-11}
& SR@15 & AT & SR@15 & AT & SR@15 & AT & SR@15 & AT& SR@15 & AT \\
\midrule 
\textbf{UNICORN} & $\mathbf{0.535}$ & $\mathbf{11.82}$ & $\mathbf{0 . 788}$ & $\mathbf{7 . 58}$ & $\mathbf{0 . 9 8 5}$ & $\mathbf{5 . 33}$ & $\mathbf{0 . 520}$ & $\mathbf{11 .31}$&\textbf{0.602}&\textbf{10.45}  \\
\midrule
(a) - RNN &0.539&11.85&0.763&7.59&0.980&5.36&0.509&11.25&0.588&10.84\\
(b) - w/o Transformer&0.478&12.17&0.733&7.78&0.958&6.18&0.470&11.62&0.545&11.23\\
(c) - w/o GCN&0.440&12.74&0.744&7.62&0.978&5.48&0.481&11.45&0.554&11.07\\
\midrule
(d) - Random Embeddings&0.310&13.31&0.665&9.24&0.905&7.66&0.196&13.95&0.220&13.55\\
(e) - FM Embeddings&0.465 & 12.26 & 0.748 & 7.68 & 0.982 &5.50 & 0.496 & 12.25&0.579&10.89\\
\midrule 
%(f) - Random Item Selection&0.328&13.07&0.682&8.89&0.88&8.02&0.219&13.81&0.229&13.52\\
%(g) - Random Attribute Selection&0.372&12.64&0.459&10.64&0.55&9.07&0.169&13.59&0.214&13.51\\
(f) - Preference-based Attribute Selection&0.467&12.33&0.712&8.24&0.978&5.74&0.489&11.60&0.569&11.06\\
(g) - Entropy-based Attribute Selection&0.507&11.96&0.756&7.63&0.978&5.71&0.502&11.33&0.585&10.69\\
(h) - w/o Attribute Selection&0.487&12.12&0.604&9.88&0.942&6.80&0.220&12.97&0.434&12.01\\
%(h) - w/o Attribute Selection&0.487&12.12&0.204&13.38&0.942&6.80&0.160&13.97&0.134&14.01\\
(i) - w/o Item Selection&0.150&13.83&0.638&8.12&0.780&9.16&0.158&13.60&0.144&13.85\\
\bottomrule
\end{tabular}
\label{ablation}
\end{table*}
\fi


Table~\ref{result} shows the performance comparison between the proposed method, UNICORN, and all baselines across five datasets. In general, UNICORN achieves significantly higher success rate and less average turn than these state-of-the-art methods, which is also comprehensively validated by the improvements on hDCG. As for the real-world E-Commerce dataset, SCPR outperforms EAR and CRM, whose performance is largely affected by the large action space in E-Commerce dataset. Despite the effectiveness of SCPR to handle the issue of large action space in CRS, its performance in such a real-world application is still restricted by the separation of its conversation and recommendation components. Our UNICORN not only enables the conversation and recommendation to be mutually enhanced during the training process, but also attains a effective sample efficiency with the proposed action selection strategies. This leads to a substantial margin from these baselines, about 18\% for SR@15, 2 turns for AT, and 30\% for hDCG. Detailed analyses can be found as follows.



\subsubsection{\textbf{Comparison at Different Conversation Turns}}

\begin{figure}
\setlength{\abovecaptionskip}{2pt}   
\setlength{\belowcaptionskip}{2pt}
\centering
\includegraphics[width=0.48\textwidth]{exp2.pdf}
\caption{Test Performance at Different Training Episodes.}
\label{converge}
\vspace{0.1cm}
\end{figure}

Besides SR@15, we also present the performance comparison of success rate at each turn (SR@t) in Figure~\ref{diff_turn}. In order to better observe the differences among different methods, we use the relative success rate (Success Rate*) compared with the state-of-the-art baseline SCPR. For example, the line of $y=0$ represents the curve of Success Rate* for SCPR against itself. Due to the space limitation and the almost perfect performance, we omit the performance comparison on Yelp dataset and only present other four datasets here. There are several notable observations as follows: (i) The proposed UNICORN substantially and consistently outperforms these baselines across all the datasets and almost every turns in the conversation session. (ii) Due to the nature of greedy recommendation approach (Abs Greedy), it may successfully hit target items at the early stage of the conversation, leading to a relatively strong performance at the first few turns, but the performance falls quickly as the turn increases. (iii) Our UNICORN achieves the most significant performance in the middle stage of the conversation, which indicates the strong scalability for different situations no matter how large the candidate action space. (iv) We can also observe that the performance of SCPR is getting closer to UNICORN at the latter stage of the conversation, as the candidate item and attribute set is getting smaller and the task becomes easier. (v) Interestingly, EAR and CRM share a similar performance as Abs Greedy in those datasets with large candidate attribute set, i.e., Yelp* and E-Commerce, indicating their policy learning is merely working when encountering a large action space.  





\subsubsection{\textbf{Training Efficiency}}


Figure~\ref{converge} shows the test performance curves of different methods. Since Max Entropy and Abs Greedy are unsupervised methods, their curves are presented as two lines for comparisons. It can be clearly observed that UNICORN is trained more stably and requires less training episodes (i.e., interaction data) to achieve a better performance than other strong baselines. Among these baselines, the curve of SCPR is the most vibrant, since it only consider the policy of when to ask or recommend, while the decisions of question-asking and recommendation are made by two separated components. As for EAR and CRM, due to the large action space in the last three datasets, there is not much performance increase during the online training process, even getting worse. The results demonstrate the efficiency and effectiveness of the proposed unified policy learning for CRS. 




\begin{figure*}
\setlength{\abovecaptionskip}{2pt}   
\setlength{\belowcaptionskip}{2pt}
\centering
\includegraphics[width=\textwidth]{case.pdf}
\caption{Sample conversations generated by UNICORN, SCPR, EAR, and CRM. Due to the space limit, we only show the conversation at the first five turns. $|V_\mathrm{cand}|$ denotes the number of candidate items at the current turn.}
\label{case}
\vspace{-0.3cm}
\end{figure*}




\subsection{Ablation Study}
\subsubsection{\textbf{Model Components}}
We first evaluate the model components for the state representation learning, including the graph-based representation learning and the sequential representation learning. The ablation studies are presented in the first part in Table~\ref{ablation} (row (a-c)). We observe that using Transformer encoder for sequential representation learning achieves slightly better performance than using RNN (row (a)), but it is not dominant. Besides, the performance on 4 out of 5 datasets suffers a larger decrease by discarding sequential learning (row (b)) than discarding graph-based learning (row (c)). We attribute this to two reasons: (i) The pretrained TransE embeddings have already encoded certain graph-based knowledge into the node representations. (ii) Since there are relatively larger number of attributes in these four datasets than LastFM, it is more important to model the interrelationships among diverse user-accepted attributes for capturing user preferences. 



\subsubsection{\textbf{Pre-training Embeddings}}
The second part in Table~\ref{ablation} (row (d-e)) presents the results that we replace pretrained TransE embeddings with randomly initialized embeddings (row (d)) and pretrained embeddings from FM model described in \citet{wsdm20-ear} (row (e)). First of all, we observe a substantial performance gap between UNICORN with randomly initialized embeddings and that with pretrained embeddings, either TransE or FM. This result shows that the pretraining is necessary and simply online training with  interactive conversations is far from efficient and sufficient for training a CRS with limited interaction data. In addition, even though UNICORN with FM embeddings still outperform other FM-based CRS, including CRM, EAR, and SCPR, using TransE embeddings can further improve the performance to a great extent, which also validates the benefits from the graph-based learning framework. 



\subsubsection{\textbf{Action Selection Strategies}}
The last part in Table~\ref{ablation} (row (f-i)) presents the results that we replace or discard the proposed action selection strategies. One alternative attribute selection strategy is to adopt the same strategy as the preference-based item selection by changing the object from items to attributes. Another one is to use the original maximum entropy function~\cite{wsdm20-ear}. The result (row (f,g)) shows that the performance of UCRPL suffers a noticeable decrease when adopting the preference-based or entropy-based strategy, indicating that it is required to consider both the user preference and the capability of reducing candidate uncertainty when deciding the asked attribute. 
Without attribute selection, we observe that the impact on applications with small action space (e.g., LastFM and Yelp) is less than those with large action space (e.g., LastFM*, Yelp*, and E-Commerce). While UNICORN is merely working without item selection, since there is no pretrained recommendation components in the framework and the preference-based item selection serves as an auxiliary item recall process. 
%Within 10,000 training episodes, the performance of UCRPL suffers a noticeable decrease when adopting random action selection strategies, which demonstrates the proposed action selection strategies preserve a remarkable sample efficiency. 

\begin{table}
\setlength{\abovecaptionskip}{2pt}   
\setlength{\belowcaptionskip}{2pt}
%\setlength{\tabcolsep}{1.5mm}{
\centering
  \caption{The impact of hyper-parameters.}
\begin{tabular}{ccccccc}
\toprule 
Dataset&\multicolumn{3}{c}{LastFM*}&\multicolumn{3}{c}{E-Commerce}\\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
$K_v$&10&20&50&10&20&50\\
\midrule
$K_p$=1&0.333&0.321&0.306&0.202&0.194&0.186\\
%$K_p$=5&0.344&0.322&0.297&0.215&0.199&0.189\\
$K_p$=10&\textbf{0.349}&0.305&0.297&\textbf{0.217}&0.205&0.189\\
$K_p$=20&0.298&0.286&0.254&0.202&0.199&0.178\\
\midrule
\midrule
$L_g$&1&2&3&1&2&3\\
\midrule
$L_s$=1&0.320&\textbf{0.349}&0.341&0.202&0.217&0.212\\
$L_s$=2&0.324&0.346&0.332&0.182&\textbf{0.221}&0.216\\
$L_s$=3&0.315&0.340&0.339&0.189&0.208&0.196\\
\bottomrule
\end{tabular}
\label{hyper}%}
\vspace{0.2cm}
\end{table}

\iffalse
\begin{table}
\setlength{\abovecaptionskip}{2pt}   
\setlength{\belowcaptionskip}{2pt}
%\setlength{\tabcolsep}{1.5mm}{
\centering
  \caption{The impact of hyper-parameters.}
\begin{tabular}{ccccccc}
\toprule 
Dataset&\multicolumn{3}{c}{LastFM*}&\multicolumn{3}{c}{E-Commerce}\\
\midrule
$K_v$&10&20&50&10&20&50\\
\midrule
$K_p$=1&0.709&0.720&0.699&0.557&0.552&0.544\\
$K_p$=5&0.805&0.741&0.663&0.597&0.591&0.577\\
$K_p$=10&\textbf{0.788}&0.739&0.652&\textbf{0.602}&0.598&0.572\\
$K_p$=20&0.738&0.641&0.572&0.600&0.594&0.568\\
\midrule
\midrule
$L_g$&1&2&3&1&2&3\\
\midrule
$L_s$=1&0.756&\textbf{0.788}&0.784&0.589&0.602&0.595\\
$L_s$=2&0.762&0.782&0.780&0.576&\textbf{0.606}&0.602\\
$L_s$=3&0.762&0.785&0.781&0.585&0.600&0.588\\
\bottomrule
\end{tabular}
\label{hyper}%}
\vspace{0.2cm}
\end{table}
\fi


\subsection{Parameter Sensitivity Analysis}
The upper part in Table~\ref{hyper} summarizes the experimental results on varying the number of selected candidate actions. Since similar conclusions can also be drawn on other datasets, we only report the results on LastFM* and E-Commerce datasets due to space limit. As for the number of selected attributes, it is likely to discard the important attributes when only selected the attribute with the highest weighted entropy (e.g., $K_p$=1). However, within a certain training interaction period (10,000 episodes in our case), UNICORN generally achieves the best performance when only selecting a small amount of candidate items for policy learning. The results also demonstrate the necessity of pruning the available actions when there is a large action search space in UCRPL. 


The lower part in Table~\ref{hyper} shows the experimental results on varying the number of network layers. AS for GCN, 1-hop aggregation is not enough for capturing all the useful information for graph representational learning. However, there is no much difference between 2-hop and 3-hop. Besides, for Transformer, we can see that 1-layer is sufficient for a good performance. 








\subsection{Qualitative Analysis}

In order to intuitively study the difference between the proposed UNICORN and other state-of-the-art CRS, we randomly sample a real-world interaction from the E-Commerce dataset. The generated conversations by UNICORN, SCPR, EAR, and CRM with the user simulator are presented in Figure~\ref{case}. Facing the large candidate action space, CRM tends to only trigger the recommendation component to make recommendations, and EAR continuously asks the questions that are not preferred by the user. Despite the success of SCPR on predicting user-preferred attributes, the policy learning in SCPR only decides when to ask or recommend, based on the number of candidate items, which leads to some unnecessary or redundant question-asking turns. UNICORN systematically addresses these issue by making a comprehensive decision of the next action. In this case, we observe that UNICORN successes to make recommendations even though there are still hundreds of candidate items, while SCPR keep asking questions until the candidate item set is small enough. 

\section{Conclusion}
In this work, we formulate three separated decision-making processes in conversational recommendation systems, including when to ask or recommend, what to ask and what to recommend, as a unified policy learning problem.
To tackle the unified conversational recommendation policy learning problem, we propose a novel and adaptive reinforcement learning framework, which is based on a dynamic weighted graph. In addition, we further design two simple but effective action selection strategies to handle the sample efficiency issue.
Experimental results show that the proposed method significantly outperforms state-of-the-art CRS methods across four benchmark datasets and the real-world E-Commerce application with a remarkable scalability and stability. 
